The Proficiency-Congruency Dilemma: Virtual Team Design and Performance in Multiplayer Online Games

Multiplayer online battle arena games provide an excellent opportunity to study team performance. When designing a team, players must negotiate a \textit{proficiency-congruency dilemma} between selecting roles that best match their experience and roles that best complement the existing roles on the team. We adopt a mixed-methods approach to explore how users negotiate this dilemma. Using data from \textit{League of Legends}, we define a similarity space to operationalize team design constructs about role proficiency, generality, and congruency. We collect publicly available data from 3.36 million users to test the influence of these constructs on team performance. We also conduct focus groups with novice and elite players to understand how players' team design practices vary with expertise. We find that player proficiency increases team performance more than team congruency. These findings have implications for players, designers, and theorists about how to recommend team designs that jointly prioritize individuals' expertise and teams' compatibility.

==> removed_content.tex <==
%\textbf{ (1. Social interaction in online games) }  \\
% - We interact with others at home, work, or in many other social situations.  \\
% - The same is true on virtual environment in online games. \\
% - When you play massively multi-player online games, you interact with other players in real time
% - To reach a goal in a game (ex) to win the game, raid a powerful mob ) with other players, you probably cooperate or compete with other players.

%\textbf{ (2. MOBA) }  \\
%  - One of the well-known type of a online game, MOBA, has both properties; cooperate with your teammates, compete with opponent teams; it is good type of the games that study the nature of intra- and inter-team interactions. \\
% - MOBA stands for match-based multiplayer online battle arena. \\
% - A player controls a single character that has various abilities in one of competing teams. \\
% - The goal that shared with team members is destroy the main structure in the enemy's base or get surrender of the opponent team. \\
% - A player can kill the units or enemy team member through interacting with other teammates to win the game. \\
% - This real-time social interaction is highly important to dominate the opponent team. \\

%\textbf{ (3. Previous Studies related to MOBA) } 
% - Then, how should we interact with teammates to enjoy the game? In other words, what behavior or team characteristic makes the game win? \\
% - In previous studies, toxic behaviors \cite{kwak_cyberbullying_2015} in LoL that may lead to lose the match have been studied; other study investigated social relations between gamers in terms of social network in Dota. \\
% - There is no study that analyzing the relation between the team performance that winning the game and individual/team characteristics in terms of online games, specifically MOBA games. \\

%\textbf{ (3. Summary)  } \\
% - In this paper, we explore the intra-player(skills) and inter-player(team composition) factors within a team affecting to the team peformance that lead a team to victory. \\
% - Through qualitative method; interviewing gamers, and quantitative method; large-scale dataset of match history of millions of players. \\
% - We expect the findings may be also applied to virtual teams in other cooperative contexts. \\

%\textbf{ (1. Traditional team research literature) } \\
% - A match can viewed as performing a competitive team task task cooperatively. \\
% - It can be analyzed based on the IPO model \\
% - input as team composition, functional diversity in champion selection in a team \\
% - process as communication, through on-line/off-line \\
% - output as team performance, win ratio \\

%\textbf{ (2. Team composition and its performance) }
% - functional diversity and team performance

%\textbf{ (3. Individual competence and its performance) }
% - Individual competence and team performance

%\subsection{RESEARCH QUESTIONS AND HYPOTHESIS}

%RQ1. How many role in a match a player can take, and what is the role? \\
	%RQ1a. What affects the selection of a role(champion) \\
	%RQ1b. When selecting the role, communication matters? \\
%RQ2. In a team, how can a functional diversity and individual proficiency of a player be measured? \\
%RQ3. Does functional diversity and individual proficiency affect the team performance? \\
%	RQ1a. Does functional diversity affect the team performance?\\
%	RQ2b. Does individual proficiency affect the team performance? \\
%	RQ3c. If two components conflicts, what decision should be made to increase team performace? \\ 
%	RQ3d. When playing the game, communication as internal process of a team matters? \\

%\section{Results}
%We test each of the three hypotheses we developed in the background section using a combination of descriptive, statistical, and qualitative methods.

%We identify 22 individual and team-related features inspired by teamwork theories discussed in the Background section. We first quantitatively formalize the team features and investigate how the feature values change from low-level to high-level teams. Than, we use all/subset of the features to predict whether a team will be victorious on a match. Finally, we explore representative features in detail and report some notable patterns.

% Our features are based on the methodology of representing champions as multidimensional vectors and calculating their distances, which is formulated in the previous section. 

% \begin{table}[]
% \centering
% \resizebox{0.45 \textwidth}{!}{%
% \begin{tabular}{l  |  l  |  r} \hline
% \multicolumn{1}{c |}{Category}           & \multicolumn{1}{c |}{Factor}  & \multicolumn{1}{c}{Ranking} \\ \hline
% \multirow{6}{*}{Indiv. Proficiency}    & proficiency\_mean           & 2       \\
%                                       & sorted\_prof\_1             & 7       \\
%                                       & sorted\_prof\_2             & 5       \\
%                                       & sorted\_prof\_3             & 3       \\
%                                       & sorted\_prof\_4             & 1       \\
%                                       & sorted\_prof\_5             & 4       \\  \hline
% \multirow{11}{*}{Functional Diversity} & in-game\_diversity          & 8       \\
%                                       & in-game\_distance\_min      & 13      \\
%                                       & in-game\_distance\_max      & 18      \\
%                                       & min\_components\_sum        & 9       \\
%                                       & max\_components\_sum        & 20      \\
%                                       & intra\_diversity\_mean      & 11      \\
%                                       & sorted\_intra\_diversity\_1 & 15      \\
%                                       & sorted\_intra\_diversity\_2 & 10      \\
%                                       & sorted\_intra\_diversity\_3 & 12      \\
%                                       & sorted\_intra\_diversity\_4 & 14      \\
%                                       & sorted\_intra\_diversity\_5 & 19      \\   \hline
% \multirow{4}{*}{Luck \& Environment}           & starting\_position          & 6       \\
%                                       & most\_pick\_diversity       & 17      \\
%                                       & most\_pick\_distance\_min   & 16      \\
%                                       & most\_pick\_diversity\_max  & 21     \\ \hline
% \end{tabular}}
% \caption{My caption}
% \label{my-label}
% \end{table}

%\begin{figure}[t]
%\centering
%  \includegraphics[width=0.7\columnwidth]{figures/adding_removing_factors.pdf}
%  \caption{Prediction accuracy using different combinations of features. Yellow bar is the prediction result using all features. Bars in adding factors represent the prediction results when only features in certain categories are used. Bars in removing factors represent the prediction results when features in the categories are removed.}~\label{fig:adding_removing}
%\end{figure}

%In most cases, team composition features, such as team diversity and team functional coverage are formed later than the features in other categories. First, team assignment features are predetermined and unchangeable for users when they are assigned to a virtual team; then, individual proficiency is players' major consideration not only because it is the most decisive factor in team performance, but also because it directly relates to their skill levels and enjoyment regarding the match. On the other hand, team composition features are determined at a team level as a collective unity, which is less prioritized for individual players. In Figure \ref{fig:adding_removing}, we observe that individual features are the most powerful when predicting team performance, followed by team assignment features and team composition features. However, we also observe that including/excluding team composition features significantly increases/decreases the win-lose prediction accuracy. 

%From the prediction results, we confirm that all three categories, individual proficiency, team composition, and team assignment, uniquely contribute to team performance. In the next section, we look at the challenging aspects of keeping the team composition features at a high level, and investigate how elite teams cope with this challenge by effective team communication.

%\section{Implicit sign of user communication observed in elite teams}
%In this section, we look at the features that collide or restrict one another, and investigate patterns of mitigating such negative correlations shown in high level teams. Finally, we conduct interviews of both low and high level players and argue that successful teams and players excel at effective communication and usage of given information than their counterparts.

%\subsection{Elite teams' traits}
%Team diversity, unlike team assignment, is controllable by team members, yet is less prioritized compared to individual proficiency values. We investigate how team diversity is associated with these two factors by conducting ordinary least squares (OLS) analysis and looking at the coefficient values of the factors as a predictor of team diversity. The patterns that support our claim is consistent for all regions. 

%\begin{figure}[t]
%	\centering
%		  \includegraphics[width=0.9\columnwidth]{figures/tier_ratio.pdf}
%		  \caption{The ratio between the 1st pick's and the 5th pick's proficiency. Solid lines are the ratios for all users and dashed lines are the ratios of the teams with bottom 10\% diversity of proficient champions. 1st pick players choose more proficient champions than 5th pick players, but this  trend less significant in higher tiers compared to lower tiers. Moreover, teams in higher tiers are less susceptible to the overlaps of the most-pick champions. The result is consistent throughout all regions.}
%		  \label{fig:tier_ratio}
%\end{figure}

%In this section, we look at how users with varying success levels react differently to the different degree of self-information disclosure levels. 

%In this section, we present the function of self-information sharing that disclosing one’s role preference and proficiency to the other team members with varying success levels.

%We constructed 2 teams for each elite and novice players, and a team played 3 matches sequentially by experimental conditions which represent three different information disclosure levels:

%\begin{enumerate}
%For both low and high-level teams, we asked the participants to select champions in three different information disclosure levels. 
%\item (No Communication) Participants have no background information of the other team members and they are not allowed to communicate with each other to understand the other teammates' proficiency levels; \vspace{-.5em}
%\item (Text-only Communication) Participants are able to communicate with each other during the champion selection procedure, only in the chatting room which is natural when playing alone; \vspace{-.5em}
%\item (Free Communication) Participants can utilize both on-line (textual) and off-line (verbal) communication to decide a role to play in a match. 
%\end{enumerate}

%Using this experimental setting, we can look at how the different degree of proficiency-overlap risk can affect participants' champion selection behavior. 

%There are 4 key findings in our experiment:
%\begin{enumerate}
%\item When information sharing is restricted, in case of elite players, their anxiety level tend to increase due to the possibility of role overlap, and they try to pick stable champions to play specific roles to reduce the risk arisen from the absent of communication. \vspace{-.5em} 
%\item When information sharing is restricted, since novice players are focusing on to champion rather than a role, they worry little about the role overlap that may result in the fail of composing a good team. In addition, they have no coping strategy of restricted communication when picking a champion. \vspace{-.5em} 
%\item When information sharing is allowed, regardless of player's tier, it tends to resolve the proficiency-diversity dilemma by generalist’s yielding a specific role to a specialist of that role, which leads to maximize mean proficiency level of a team with preserving the functional diversity of a team. \vspace{-.5em} 
%\item The information sharing process tends to be more efficient to resolve the dilemma in the case of experts while lower tier players suffered insufficient time to do it.
%\end{enumerate}

%Interestingly, elite players are comfortable to relieve the dilemma in limited amount of champion-picking time when they are allowed to communicate with each other in Text-only and Free Communication conditions, but novice players are not. A Silver 5 player P19 reported:

%\begin{quote}\textit{
%"I thought that we should have talked more about each other before playing the games... we didn't decided where (which lane) to go before, so I was nervous of picks of teammates and opposing team... I hurried to select a champ." (P19)
%}\end{quote}

%In conclusion, information sharing is helpful to resolve proficiency-diversity dilemma suffered by players and it leads to maximize mean proficiency level of a team with preserving the functional diversity of a team. In addition, The process is natural and more efficient in elite teams while novice teams are not. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this section, we show the perception of a role in a team that of LoL players. There are 2 key findings in the interview:

%\begin{enumerate}
%\item There are 5 distinctive roles in a team. 5 roles need to be assigned for each team members. There is a role not assigned to anyone in a team; that is, there should be no overlap of a role between team members.  \vspace{-.5em} 
%\item The basic comprehension of these roles are immediately acquired when a player enjoyed the game for a first few times. As a player's gaming experience accumulated to get higher tiers, the degree of understanding the roles are developed. Moreover, elite players are sensitive about the current \textit{"meta"} (trend) which includes popular champion picks for each roles, style of game operation.
%\end{enumerate}

%A team is composed of 5 players who should take a role among followings: \textit{Top, Mid, AD-carry, Supporter} and  \textit{Jungle}. According to what distinctive role a player have taken, player's in-game behavior and expectation of the other teammates also may be different.

%First, \textit{"Top"} appears in the top lane, as in Figure~\ref{fig:map}. \textit{"Top"} should protect teammates and endure enemy's attacks during a battle. \textit{"Top"} should also bother opponent \textit{"Mid"} or \textit{"AD-carry"} to interrupt them attacking teammates, if possible. 

%\begin{quote}\textit{
%"I think having [crowd control] skills and doing tanks is important to the Top, As a main tank of a team, Top should bruise the enemy damage-dealers..." (P2)
%"Top must be tank, just... protecting our Mid and AD-carry as best I can is critical " (P16)
%}\end{quote}

%Next, \textit{"AD-carry"} and \textit{"Supporter"} goes to the bottom lane. \textit{AD-carry} attacks enemy champions at a distance with \textit{physical} damage by auto-fires. It is specialized in damage-dealing that possesses most powerful attack power in a team. Supporter mainly supports the AD-carry's growth.

%\begin{quote}\textit{
%"AD-carry attacks at a long range. It must deal great amount of damage, and Supporter raise AD-carry to do it. However, if it can't do that pretty well, it's a failure... When the match ends, It must have dealt heaviest damage to opponents in a team. Basically, It most deals a damage in the latter part of the match... Supporter is a role that helps AD-carry to get stronger. (differ from AD-carry) defensive skills are crucial, healing skills are also very important... (nowadays) Braum or Alistar is popular picks." (P1)
%}\end{quote}

%Fourth role is \textit{"Mid"} which takes the mid lane. Similar to \textit{AD-carry}, \textit{"Mid"} deals a significant amount of damages to opponents yet using its attack skills. Also, It should help top or bot lane players as a patrol.

%\begin{quote}\textit{
%"First of all, killing CS with not missing it(auto-spawned AI units called Minion that you can get some golds and experience points if they are killed) is crucial as a AD-carry, the different part is AD-carry must farm continuously but Mid should patrol around to other lanes. Mid must roam bot to top after dominating opponent Mid and destroy the tower..." (P12)
%}\end{quote}

%Lastly, \textit{"Jungle"} does not appear on any lanes in the beginning part of a match. They hunt AI units in Jungle area, and they perform surprise attacks with teammates to kill the opponent lane players. Moreover, they read a whole map with expanding the vision of a team.

%\begin{quote}\textit{
%"Jungle should manage the objects... Sometimes, Jungle need to protect the towers... If Supporter is trying to ward, Jungle must help it and remove the opponent's ward at the same time. In addition, you must care about opponent's diving to our tower or teammates diving into opponent's tower... A Jungle must keep all of the lanes in mind always, so it's hardest role in a team, sometimes annoying... you should not miss the timing, always " (P7)
%}\end{quote}

%These five roles are immediately acquired when a player enjoyed the game for a first few times. A player learns what they have to do in the game by friends or other players. As their game experience accumulates, they construct deeper comprehension of the roles.

%\begin{quote}\textit{
%"When friends invited me to the game for the first time, my friends taught me as if it was a rule." (P19)
%"Professional gamers do like that." (P2)
%"If you don't go (to the lane) where you have to go, you will suffer from disadvantages... For example, a opponent is shooting on you at a distance, but there will be nothing more you can do." (P1)
%}\end{quote}

%If a player is not aware about the implicit rules related to each roles, the player is criticized by teammates. A role that assigned to each player should be performed well is a norm between players:

%\begin{quote}\textit{
%"If you go to other lane (that you should not go to), you will be criticized, and you will learn about it." (P2)
%"There is a atmosphere, if you violate it and insist go to top lane while you are a Supporter, teammates will swear at you." (P4)
%}\end{quote}


